Context Aware Query Rewriting for Text Rankers using LLM

Query rewriting refers to an established family of approaches that are applied to underspecified and ambiguous queries to overcome the vocabulary mismatch problem in document ranking. Queries are typically rewritten during query processing time for better query modelling for the downstream ranker. With the advent of large-language models (LLMs), there have been initial investigations into using generative approaches to generate pseudo documents to tackle this inherent vocabulary gap. In this work, we analyze the utility of LLMs for improved query rewriting for text ranking tasks. We find that there are two inherent limitations of using LLMs as query re-writers -- concept drift when using only queries as prompts and large inference costs during query processing. We adopt a simple, yet surprisingly effective, approach called context aware query rewriting (CAR) to leverage the benefits of LLMs for query understanding. Firstly, we rewrite ambiguous training queries by context-aware prompting of LLMs, where we use only relevant documents as context.Unlike existing approaches, we use LLM-based query rewriting only during the training phase. Eventually, a ranker is fine-tuned on the rewritten queries instead of the original queries during training. In our extensive experiments, we find that fine-tuning a ranker using re-written queries offers a significant improvement of up to 33% on the passage ranking task and up to 28% on the document ranking task when compared to the baseline performance of using original queries.

==> 02-query-modelling.tex <==



\section{Impact on query modelling}
\label{sec:query-modelling}

The brevity of search queries and the potential ambiguity of user intent pose challenges for search systems to retrieve relevant documents. Search systems apply a wide variety of techniques to address this issue~\cite{chang2020query}. In this section, we delve into the query understanding and rewriting methods commonly used in retrieval tasks and conversational settings.

\vspace{-2.5mm}
\subsection{Query Understanding for Retrieval}
One of the basic techniques in query understanding is use of query classification to identify the target topic~\cite{beitzel2005improving} to retrieve relevant documents to the topic. Intent classification is another popular method for which several taxonomies and models to classify the query intent have been proposed~\cite{broder2002taxonomy,rose2004understanding,baeza2006intention}. Another common problem is spelling correction in queries commonly solved by edit distance~\cite{shang1996tries} and probabilistic approaches~\cite{li2012generalized}. While these methods improve query understanding, they are not align the user intent with the query in a scrutable way.

The goal of query rewriting is to align the query with the user intent. Both shallow and deep neural models are proposed for the query rewriting. Shallow models use substitution-based methods, which replace the query by substituting terms and phrases with synonyms and related phrases~\cite{jones2006generating}. A closely related method is query expansion, which adds relevant terms using the pseudo-relevance feedback~\cite{lv2009comparative}.  More modern approaches use word embeddings to rewrite queries~\cite{grbovic2015context}. There are also generative models which use Seq2Seq models~\cite{he2016learning} and reinforcement learning for generating rewritten queries~\cite{nogueira2017task}. Auto-completion and query suggestions are ways to guide the user to resolve the query intent more iteratively. There is a rich literature which suggests that these methods improve search performance~\cite{baeza2004query}. Unlike these methods, which rewrite the queries as keyword queries, our work focuses on generating natural language queries which are faithful and scrutable to the user intent.

Natural language question generation for query understanding is a relatively new trend in IR. \cite{rao2018learning} introduced a model to generate questions that clarify missing information in a specific setting. They used a reinforcement learning model to maximize a utility function based on the value added by the potential response to the question. \cite{trienes2019identifying}, on the other hand, focused on identifying unclear posts in a community question answering setting that require further clarification. While these methods are domain-specific, \cite{zamani2020generating} propose using template-based slot-filling using both weakly supervised and reinforcement learning for open domain IR. Generating clarifying questions is more commonly used in conversational setting, which we discuss further in Section \ref{subsec:conv}. 

Although the methods mentioned above enhance the comprehension of queries, they cannot always substitute for one another, and combining them in sequential manner in search systems can introduce errors retrieving information. Our goal is to minimize the number of components in search systems for capturing the user query intent by natural language intent generation.

\subsection{Conversational Query Understanding}
\label{subsec:conv}

Conversational query rewriting is aimed at transforming a brief, context-dependent question into a fully specific, context-independent query that can be processed effectively by existing question answering and information retrieval systems. \cite{elgohary2019can}~introduced the task of conversational query rewriting with the CANRAD dataset, with the goal of making the queries self-contained. Several approaches exploit this dataset to improve the performance of conversational settings. \cite{vakulenko2021question}~propose a generative approach to replace tokens in the question to make it context-independent. Another approach uses few-shot fine-tuning of LLMs to generate queries that improve conversational search performance~\cite{yu2020few}. Others like ConQRR (Conversational Query Rewriting) rewrite a conversational question in context into a standalone question using a novel reward function to optimize retrieval models directly via reinforcement learning~\cite{wu2021conqrr}. These methods mainly focus on resolving co-references of pronouns, which is complimentary to the our approach in which we need to infer query intent from limited context.

Query suggestion is another way to guide users towards the right query in a conversational setting~\cite{rosset2020leading, sordoni2015hierarchical}. Asking clarifying questions is widely used for query understanding in conversational settings, which allows the users to provide additional context~\cite{bi2021asking, zamani2022conversational}. While these methods need training data resulting in cold start problems, \cite{wang2023zero} introduce zero-shot clarifying question generation.

Our approach does not rely on conversation context or prior answers, and instead works with under-specified queries to align human intent with machine intent.
%% do some pronoun resolution, they are complimentary approach. Get the context correct we want to understand the latent intent.


% \subsection{Scrutable Query Rewriting}

% In information retrieval, query expansion is adding additional terms to a user's search query to improve the search results' precision or recall. 
% Traditional approaches add synonyms, related terms, and concepts to the original query using a thesaurus or a knowledge base.
% Query expansion can be a valuable tool for improving the accuracy and relevance of search results, particularly in cases where the original query is too broad or ambiguous. 
% However, it is essential to use query expansion carefully, as it can also lead to irrelevant or unrelated results due to topic drift.


% Closely related, \textit{query rewriting} refers to modifying a user's search query to improve the quality of the search result. 
% Like query expansions,  rewriting can be also be done by adding additional terms to the query. Still, unlike expansions it involves removing unnecessary terms, or reordering the terms in the query.


% \subsection{Machine Translation in IR}

% Statistical machine translation (SMT) has been explored in detail for IR where we consider queries as texts in one language and documents as texts in another. Retrieval by translation models is a family of supervised approaches that aim to learn translation probabilities from queries to associated relevant documents obtained from labeled training data.

% Machine translation methods have been used as a discriminative model to judge \texttt{<query, doc>} relevance~\cite{gao2010clickthrough:mt:discriminative} or to improve query re-writing~\cite{wang2020deep:query:rewrites}.



\subsection{Large Language Generative Models}

Recent advances in neural text generation have demonstrated that large language models (LLMs) trained in a self-supervised generative fashion generalize well to downstream tasks in a few-shot or zero-shot setting \cite{brown2020language, wei2021finetuned, alayrac:2022:flamingo}. 

Prompting is shown to be an effective way for controlled text generation, zero-shot and few-shot learning of downstream tasks. In dense retrieval, Hyde \cite{hyde} demonstrates impressive zero-shot performance. The approach instructs a prompt based language model like \textsc{InstructGPT} to generate a hypothetical document followed by a dense retriever \cite{contriever} which introduces a bottleneck aiding to retrieve relevant documents. Our approach is unsupervised and requires no training and supervision in the form of relevance scores.

\subsection{Minimize Hard Query Rewrites}
We argue that query rewriting, whether in traditional IR or a conversational setting, provides limited flexibility to users. Despite the availability of several tools in existing search systems to capture query intent, users still need to rewrite their queries, resulting in hard rewrites as mentioned in Section \ref{sec:hard-rewrites}. Therefore, we propose the following research direction:

\mpara{RD I (Minimize Hard Rewrites):} \textit{How can we align machine intent with human intent while minimizing the need for hard query rewrites by the user?}

Current query rewriting methods spread tools across multiple components, making them less efficient for users. Our proposed solution is a single query rewriter that uses LLMs to create natural language query descriptions from vague keyword queries. These descriptions provide users with a clearer understanding of the machine's intent, enabling them to make more informed decisions and reducing the need for extensive hard query rewrites.

One of the challenges in RD I is to evaluate the effectiveness of the different modes of query rewriting mentioned in Section \ref{sec:feedback}. One way to assess scrutability is to use quantitative measures, such as evaluating how often the user commits to the query rewrite over soft rewriting and hard rewriting. 

==> 03-perspective-interpretability.tex <==
\newcommand{\rewriter}{LLM}

\section{Impact on Explainable Rankers}
\label{sec:perspective-interpretability}

In the area of explainable IR, the central goal is to explain the reasoning behind the ranking decisions made by a ranker using an \textit{explanation} that is \textit{faithful} to the ranking model~\cite{anand2022:exir}.
Explanations are user-centric and can have multiple forms e.g., heatmaps or \textit{feature attributions}, extractive text snippets or \textit{rationales}, and term-based~\cite{singh:2020:fat:intentmodel,lyu:ecir:23:multiplex}. 
In some sense, most of EXIR approaches either directly~\cite{singh:2020:fat:intentmodel,lyu:ecir:23:multiplex} or indirectly~\cite{verma:2019:sigir:lirme,polley:2021:exdocs} try to uncover the often latent machine intent. 
Consequently, the natural language \mi{} from the \rewriter{} can naturally serve as an \textit{explanation} of the downstream ranking task if it is \textit{faithful} to the underlying ranking model.
The concept of faithfulness or fidelity is an important and necessary condition for explainers.
It refers to the ability of the explanation to truly capture the true behavior of the ranking model.
An explanation can be plausible or human understandable, even persuasive and convincing, but is not faithful to the ranking model if the ranker uses a different reasoning (different features, text patterns, shortcuts) for ranking. 

\subsection{Research Context}
% \subsection{Overview of Explainable IR}

Full interpretability while ensuring competitive performance is often hard, if not impossible, to attain with neural architectures. 
However, there has been progress in the area of explainable IR that are either \textit{interpretable-by-design} or \textit{posthoc methods}~\cite{zhang:2021:wsdm:expred,lei:2016:emnlp:rationalizing,leonhardt2021learnt}.
Posthoc methods for interpretability do not trade-off model performance for interpretability and are employed after model a ranking model is trained to posthoc analyse the reasons for the prediction. 
Unfortunately, most of the explanations of the posthoc methods are term-based and hence not fully specified for the end user.


More importantly, such methods are not entirely faithful to the trained ranking models. 
Moreover, it is also hard to evaluate if these models have faithfully deciphered the machine intent of the ranking models.
Models that are entirely faithful and provide a better specification of the query intent are explain-then-predict models. 
These models deliver partial interpretability using rationale-based explanations as an intermediate step. 
However, their explanations are not \textit{scrutable} and are limited to extractive pieces of text from documents in the ranked list. 

\input{tables/table-interpretability}


It is still the prerogative of the user to decipher the machine intent from the multiple (query, document) explanations. 
Our framework intends to build ranking models that are \textit{interpretable-by-design} where the machine intent can be fully specified in natural language for the user to scrutinize.


~\cite{radlinski2022natural} contrast the current approach of blackbox user models in recommender systems with a proposed scrutable user modeling allowing control of a system’s personalization.
Scrutable user models represent user models in natural language (NL) where scrutable language is defined as being both short and clear enough for someone to review and edit directly. Table ~\ref{tab:datasets} compares  different approaches based on \textbf{Plausible}, \textbf{Quality}, \textbf{Faithful} and \textbf{Editable} dimensions.


\begin{itemize}
    \item \textbf{Plausible or Human understandable:} Posthoc interpretability ~\cite{singh:2020:fat:intentmodel,fernando:2019:sigir:studyshaponretrieval,singh:2019:wsdm:exs}. High on understandability but low on plausibility.

    \item 
    \textbf{High performance:}
    posthoc methods are high on performance. Expred models trade-off performance and sparsity (plausibility)~\cite{leonhardt:2021:arxiv:hard:kuma:ranking,zhang:2021:wsdm:expred}. Expred models might not be high performance.

    \item
    \textbf{Faithful} Not only plausible. 
    Posthoc methods are plausible but not faithful. Expred models are fully faithful.

    \item
    \textbf{Scrutability.}
    Neither expred nor posthoc methods are scrutable. 
    CQA, e-cos, NLI datasets looked at generative models so they might be scrutable.
    
\end{itemize}


\subsection{Machine Intents as Explanations}

The primary question for realizing an interpretable machine intent is to make sure it is faithful to the model decision.
Towards this we define the following research direction:

\mpara{RD II (Faithful Machine Intents):} \textit{How do we ensure highly faithful \mi{} to the ranking model, while still being plausible and retaining good ranking performance.
}

A simple yet popular solution is to follow a \textit{rewrite-then-rank framework}  where a generative model is first trained to generate query explanations or query descriptions from an under-specified query. 
Subsequently, a neural ranker is trained to leverage the generated query explanation to retrieve relevant documents from the corpus.
To respect the faithfulness criterion, interpretability constraints have to be imposed over end-to-end training regimes.
Recently, proximal-policy optimization approaches~\cite{rlhf,ppo} have been proposed to train such chained models with arbitrary rewards. 
Rewards measuring the fidelity between intents and rankings can then be used to train both the rankers and the rewriters.
For example for the query ``Panther showtimes'' the generative LM generates ``Show the time slots for panther visit in local zoo''. But based on a scalar reward (human feedback) judging the relevance of returned documents the generator could rewrite the query intent to ``Show the time slots for black panther movie in theatre''.

% \begin{itemize}
%     \item Can we generate query explanations that cover various aspects of the query? Can we leverage existing query-intent pairs data for this task?

%     \item Can we build a retriever that operates on the outputs from the first stage query explanation generator to retrieve relevant documents?

%     % \item Can we leverage feedback of the relevance of documents to fine-tune the retriever and the generator aiding the generator to generate better query explanations? Do we use a RL framework for this purpose?
% \end{itemize}



\subsection{Rationale-based Models}

Rationale-based models in natural language processing (NLP) and IR are machine learning models designed to generate human understandable explanations or justifications for their predictions or decisions. 
Rationale-based models typically consist of two components: a rationale-generation model and a task model. 
Given the text input, the rationale-generation model generates an extractive or abstractive explanation. The task model subsequently uses just the generated explanation to make a prediction. The task model and the rationale generation module can be trained together or in a pipelined manner, depending on the specific application~\cite{expred}.
Rationalization in NLP was first introduced in 2007~\cite{zaidan2007using} with the objective of using annotator rationales to improve task performance for text categorization. 
Interestingly, explainability was not the core objective. However, explainability is an advantage of rationalization because it makes the model inherently explainable even if used in the context of task improvement.
~\cite{rajani2019explain} developed the Commonsense Auto-Generated Explanations (CAGE) framework for generating explanations for Commonsense Question Answering (CQA). We envision a LLM-based query rewriter to create more accurate, transparent, and controllable ranking models. 


==> 04-perspective-training.tex <==

\section{Impact on Training Data and Model Training}
\label{sec:training-data}


Observational data collected from user clicks by modern search systems can serve as a valuable resource for training learning-to-rank (LTR) systems. However, it is widely recognized that implicit feedback through clicks may not necessarily indicate absolute relevance, particularly in LTR systems.
Click data is inherently biased, which can result in sub-optimal performance for ranking systems if left unaddressed. Indirect feedback can introduce several biases, including position bias~\cite{wsdm2017-joachims:position-bias}, trust bias~\cite{www2021-zheng:trust-bias}, selection bias~\cite{www2020-ovaisi:selection-bias} and exposure bias~\cite{sigir2016-wang:exposure-bias}, among others.
Biases tend to favor higher-ranked search results, which may receive more clicks from users, even if those results are not the most suitable for the users search query. 

The biases introduced by click data in search engines can have several negative consequences for both users and search engine providers. Biased search results can lead to a poor user experience, with users unable to find the information they are looking for, or being presented with irrelevant or low-quality results. Additionally, biased search results may reduce the diversity of results, reinforce stereotypes and biases, reduce competition, and erode user trust in search engines. 
% Therefore, it is crucial for search engine developers and researchers to address these biases through careful design, evaluation, and testing. 

We argue that our framework of collecting direct feedback data on interactive query understanding, to a large extent, reduces the over-dependence on click data and therefore substantially reduces some of the known biases.

% By doing so, search engines can provide more objective, diverse, and relevant search results that enhance the user experience and improve the reputation of search engines.


\subsection{Direct feedback from user interaction}
\label{sec:direct-feedback}

Unlike indirect feedback, direct methods for obtaining feedback from users involve relevance-feedback approaches~\cite{relevance_feedback}, where users are asked to evaluate search results and indicate which ones are relevant to their query. 
The first consequence of such direct feedback is that it useful to refine the search query and improve the accuracy of future search results. 
Current methods for direct feedback are query autocompletions~\cite{baeza2004query}, and query suggestions~\cite{rosset2020leading, sordoni2015hierarchical}, are both compatible and complementary in our intent generation framework.
% are also used to improve the relevance of future search results and provide personalized search results to the user. 
However, it should be noted that both these approaches are not (a) fully specified natural language or (b) not easily editable by the user.
% Query suggestions, on the one hand are similar queries issued by other users that are also underspecified. 
% On the other hand expansions are also term based and not free-text explanations of the machine intent. 
% Our \mi{}'s on the other hand, are fully formed descriptions that are editable. 
To reduce query abandonment and promote user interaction in the query understanding phase, the presented machine intents must attempt to diversify over the intent space.
Diversification over the intent space in not new to IR, and has been extensively researched in the context of search rankings~\cite{xquad}.
However, we propose a research direction to obviate the need for hard rewrites. 
The user can thereafter interact and provide feedback through soft rewrites as discussed in Section~\ref{sec:framework}. 
Note that on one hand, the key challenge is to first learn a diversification strategy to avoid hard re-writes and abandonment.
On the other, provide generic \mi{}s increases the number of interactions until the final commit thereby potentially causing user fatigue.
Therefore a key challenge is to  balance specialization to capture intents close to user intent with diversification. 


\mpara{RD III (Diverse Machine Intents):} \textit{How do we generate \mi{} that are diverse enough to capture possible intents for ambiguous queries? 
How do we balance diversification with specialized intents for user satisfaction?
}

Though diverse query intents are possible through a myriad of approaches ensuring that they are informative and useful for feedback is a challenge. Existing diversification methods in IR literature can be divided into \textit{implicit} and \textit{explicit} diversification methods. Implicit diversification approaches like MMR \cite{mmr} do not consider query intents and only rely on document dissimilarity. However, explicit diversification methods like xquad \cite{xquad} consider query suggestions as query aspects and ensure that atleast one relevant document for each aspect is retrieved. Potential solutions include leveraging diversification metrics to curate the training set where the query reformulations cover diverse aspects of ambiguous queries.
 

\subsubsection{Types of user-feedback data}
\label{sec:types-feedback-data}

User interaction with machine intents can provide a rich and nuanced source of data for improving information retrieval and natural language processing systems. There are several ways in which user interaction can inform and enrich this data. Firstly, when users agree with the machine intent that has been extracted, the user intent is described in near-complete detail. This can provide valuable information for developing and optimizing natural language understanding systems. Secondly, edited intents are a class of partial intents that represent small deviations from the actual intent. These deviations may reflect subtle differences in how users express themselves, which can provide insights into variations in language use and improve the robustness of natural language processing systems. Finally, query reformulations can serve as signals for non-relevance, and hence, clear negative feedback on the machine intents that are being presented.

The different types of training data that are generated through user interaction with machine intents can provide new research avenues for optimizing natural language processing systems. By minimizing the gap between machine and user intents, these systems can provide more accurate and relevant search results and improve the overall user experience. 

% \subsection{Impact on training rankers}

One of the immediate impacts of using \mi{} as queries is that it can eliminate the challenge of dealing with underspecified queries. This is because \mi{} can provide a more complete and specific representation of the user's information needs. This can have several benefits for improving information retrieval systems. For instance, it can make it easier to train transformer-based rankers between pairs of text that are more or less fully specified rather than relying on underspecified queries that are prone to ambiguity and uncertainty. 
Additionally, using \mi{} as queries can make it easier for models to compute direct answers to user queries, as they can provide more accurate and specific information on what the user is searching for. 

\mpara{RD IV (Jointly training the Rewriter and the Retriever):} \textit{How do we train the rewriter and the retriever using the feedback signals so they can mutually reinforce each other?
}

As is a common practice in moder IR systems, the re-writer and ranker can be organized in a sequence and can be trained in a pipelined or jointly.
Training such models that have a purely a natural language interface between modules is new.
For rationale-based models, both pipelined~\cite{expred}, and joint training regimes~\cite{lei:2016:emnlp:rationalizing,yoon:2018:iclr:invase} have been proposed.
However, these approaches are implemented through masking the original feature space, and therefore do not induce a fully natural language interface.
However, policy gradient based reinforcement learning with human feedback approaches \cite{ppo, rlhf} could be employed  for jointly training the re-writer and retriever.
This way, not only can we ensure the framework can directly be optimized for arbitrary losses intended metric than a loss which acts as a proxy. 
% This training regime would help in bridging the gap between machine and user intents. 
% It woudl also aid in generating faithful intents without compromising on retrieval performance.



==> tables/table-anecdotal.tex <==

\begin{table*}
    \centering
    \scriptsize
    \begin{tabularx}{\textwidth}{crl}
        \toprule
        \multicolumn{2}{r}{\textbf{Queries}} & \textbf{Intents} \\
        \midrule
        \multicolumn{3}{l}{\textbf{Query}: \texttt{Commodore}}\\
        \cmidrule{1-2}
        \parbox[b]{0pt}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Intents}}}
        & \bf 1 & A commodore's ship is typically designated by the flying of a Broad pennant, as opposed to an admiral's flag. \\
        & \bf 2 & \green{Commodore is a naval rank used in many navies that is superior to a navy captain, but below a rear admiral.} \\
        & \bf 3 & It is sometimes abbreviated: as "Cdre" in British Royal Navy, "CDRE" in the US Navy [...] \\
        & \bf 4 & Commodore (rank). \\
        & \bf 5 & Non-English-speaking nations often use the rank of flotilla admiral or counter admiral [...] \\
        \midrule
                \bottomrule
    \end{tabularx}
    \caption{Example EXAMPLE TABLE TO CONTAIN examples...\green{highlighted}.}
    \label{tab:fever_examples}
\end{table*}


==> tables/table-examples_diff_rewrites.tex <==
\begin{supertabular}{llp{.70\textwidth}}
    \toprule 
    \textbf{Method}  & \textbf{Query id}    & \textbf{query text} \\
\midrule 
Original & 127392 & define sri \\
\vinci{} & 127392 & Sri is a Sanskrit word meaning “holy” or “auspicious.” It is often used in Hinduism as an honorific title for a deity or spiritual teacher. It is also used in Buddhist and Jain contexts, and is an important concept in South Asian culture. \\
\vinci{} (doc context) & 127392 & What is the meaning of Sanskrit word "Sri" and how is it used as a title of veneration? \\
ChatGPT & 127392 & Find the definition and meaning of the acronym SRI (Socially Responsible Investing). \\
\chatgpt{} (doc context) & 127392 & What is the meaning of the Sanskrit word "Sri" and how is it used in Indian subcontinent? \\
\midrule 
Original & 97047 & coniferous herbivore \\
\vinci{} & 97047 & Find information about coniferous herbivores \\
\vinci{} (doc context) & 97047 & What health concerns have been found in the coniferous forest that are of particular concern for spotted owls? \\
ChatGPT & 97047 & What types of animals feed on coniferous trees and how do they adapt to this diet? \\
\chatgpt{} (doc context) & 97047 & What kind of herbivores can be found in the coniferous forest? \\
\midrule 
Original & 57978 & cadaver tomb \\
\vinci{} & 57978 & Find information about cadaver tombs. \\
\vinci{} (doc context) & 57978 & What is a gisant and how does it relate to cadaver tombs? \\
ChatGPT & 57978 & What is a cadaver tomb and what is its historical significance? \\
\chatgpt{} (doc context) & 57978 & What is a cadaver tomb and what is its significance in the later Middle Ages? \\
\midrule 
Original & \textbf{181039} & ephesians 6:5-9 \\
\vinci{} & 181039 & Find information about Ephesians 6:5-9. \\
\vinci{} (doc context) & 181039 & 7 With good will render service, as to the Lord, and not to men, 8 knowing that whatever good thing each one does, this he will receive back from the Lord \\
ChatGPT & 181039 & What is the meaning and interpretation of Ephesians 6:5-9 in the Bible? \\
\chatgpt{} (doc context) & 181039 & How does the passage in Ephesians 6:5-9 instruct slaves to behave towards their masters? \\
\midrule 
Original & \textbf{480437} & price nrz \\
\vinci{} & 480437 & Find information on the Pricing of Non-Recourse Z-Bonds. \\
\vinci{} (doc context) & 480437 & What is the pricing of New Residential Investment Corp. common stock on Jan 30, 2017 7:16 PM EST? \\
ChatGPT & 480437 & Find information on the pricing strategy for non-return-to-zero (NRZ) encoding. \\
\chatgpt{} (doc context) & 480437 & What is the public offering price of New Residential Investment Corp.'s common stock? \\
\midrule 
Original & 1081897 & zeigarnik effect \\
\vinci{} & 1081897 & Find information about the Zeigarnik effect. \\
\vinci{} (doc context) & 1081897 & What are the implications of the Zeigarnik effect in Gestalt psychology? \\
ChatGPT & 1081897 & What is the Zeigarnik effect and how does it affect memory recall? \\
\chatgpt{} (doc context) & 1081897 & How does the Zeigarnik effect relate to memory retention and incomplete tasks? \\
\midrule 
Original & \textbf{525248} & tty number \\
\vinci{} & 525248 & Find information about how to locate a TTY number. \\
\vinci{} (doc context) & 525248 & What is the TTY number for Disability Services? \\
ChatGPT & 525248 & What is a TTY number and how is it used for communication? \\
\chatgpt{} (doc context) & 525248 & What are the TTY numbers for Ball State University's Switchboard and Disability Services office? \\
\midrule 
Original & 389096 & hs worms \\
\vinci{} & 389096 & Find information about heartworms in dogs. \\
\vinci{} (doc context) & 389096 & What are the courses offered by Hochschule Worms? \\
ChatGPT & 389096 & Find information about the symptoms, causes, and treatment of heartworm disease in dogs. \\
\chatgpt{} (doc context) & 389096 & What are the programs offered by Hochschule Worms? \\
\midrule 
Original & \textbf{89308} & ccm requirements\\
\vinci{} & 89308 & Find information about the requirements to become a Certified Case Manager (CCM).\\
\vinci{} (doc context) & 89308 & What educational qualifications and/or experience are required to become a Certified Construction Manager (CCM)?\\
ChatGPT & 89308 & What are the requirements for implementing a critical care management (CCM) program?\\
\chatgpt{} (doc context) & 89308 & What are the requirements to become a Certified Construction Manager (CCM)?\\
\midrule 
Original & 205430 & hornworms moth \\
\vinci{} & 205430 & Find information about the hornworms moth. \\
\vinci{} (doc context) & 205430 & What is the color and wing spread of the tomato hornworm moth? \\
ChatGPT & 205430 & What is the life cycle of hornworms moth and how do they affect crops? \\
\chatgpt{} (doc context) & 205430 & What is the appearance of an adult hornworm moth? \\
\midrule 
Original & 475948 & player is \\
\vinci{} & 475948 & Find information about the Player Is project. \\
\vinci{} (doc context) & 475948 & What types of players are involved in football, video games and other sports? \\
ChatGPT & 475948 & Find information about a player, including their stats, team history, and accomplishments. \\
\chatgpt{} (doc context) & 475948 & What are the different meanings of the term "player", including Football player, Gamer, Player character, Player-coach and Player \\
\midrule 
Original & 176525 & dunn effects \\
\vinci{} & 176525 & Find information on the effects of Dunn's law. \\
\vinci{} (doc context) & 176525 & What are the features of the Dunn O Effects Nyarlathotep distortion pedal? \\
ChatGPT & 176525 & Find information on the effects of Dunn's multiple comparison test in statistical analysis.\\
\chatgpt{} (doc context) & 176525 & What are the Dunn O Effects and how are they related to the Nyarlathotep distortion pedal? \\
\midrule 
Original & 186773 & figure pitch \\
DaVinci & 186773 & Find information about how to craft a successful pitch for a business figure. \\
\vinci{} (doc context) & 186773 & What is the method for figuring roof pitch? \\
ChatGPT & 186773 & Find information on what is meant by figure pitch and its significance in aircraft design. \\
\chatgpt{} (doc context) & 186773 & What is the method used by contractors and roof framers to figure a different pitch, or any roof pitch? \\
\midrule 
Original & 1168697 & urodeum function \\
DaVinci & 1168697 & Find information about the function of the urodeum in the digestive system \\
\vinci{} (doc context) & 1168697 & What is the purpose of accessory bladders or bursae in aquatic turtles? \\
ChatGPT & 1168697 & What is the function of the urodeum in avian anatomy? \\
\chatgpt{} (doc context) & 1168697 & What is the function of outpouchings from the lateral urodeal wall in aquatic turtles? \\
\midrule 
Original & 9631 & aam designation \\
DaVinci & 9631 & Find information about AAM (Advanced Accreditation Member) designation \\
\vinci{} (doc context) & 9631 & What is the process for obtaining the AAMS designation? \\
ChatGPT & 9631 & What does the AAM designation stand for and what are its requirements? \\
\chatgpt{} (doc context) & 9631 & What is the College for Financial Planning's Accredited Asset Management Specialist (AAMS) designation? \\
\midrule 
%\end{tabular}
%\caption{Comparing rewrites of ambiguous queries using \chatgpt{} and \vinci{} model with in-context and doc-context techniques.}
%\label{tab:rewriter_all_model_example_1}
\end{supertabular}


==> tables/table-qualitative.tex <==
\begin{table*}
\begin{tabular}{l|l|p{12cm}}

\hline
\textbf{Method }                          & \textbf{topic}      & \textbf{rewrite}                                                                                                                 \\ \hline
\multirow{3}{*}{Gpt3 in context} & EPIC study          & Find information regarding EPIC (European Prospective Investigation into Cancer and Nutrition) findings on lymphoma.             \\ \cline{2-3}
                                 & Crib death          & Find information about the causes of Sudden Infant Death Syndrome (SIDS) or crib death.                                          \\ \cline{2-3}
                                 & Alli                & Find information about Alli, an over-the-counter weight loss drug.                                                               \\ \hline
\multirow{3}{*}{BART}            & EPIC study & Find information on EPIC study                                                                                        \\ \cline{2-3}
                                 & Crib death          & Find information about the Crib death bed at the NIH Medical Center.                                                             \\ \cline{2-3}
                                 & Alli                & Find information about the Alli movie, Star Trek: Voyager.                                                                       \\ \hline
\multirow{3}{*}{GPT (prompt1)}   & EPIC study          & The EPIC Study was a clinical trial that evaluated the safety and efficacy of a new investigational drug.                        \\ \cline{2-3}
                                 & Crib death          & Crib death, also called sudden infant death syndrome (SIDS), is the sudden, unexplained death of a baby younger than 1 year old. \\ \cline{2-3}
                                 & Alli                & Is Alli is a go-getter.                                                                                                          \\ \hline
\multirow{3}{*}{Gpt3 (prompt2)}  & EPIC study          & What is EPIC study?                                                                                                              \\ \cline{2-3}
                                 & Crib death          & What is crib death ?                                                                                                             \\ \cline{2-3}
                                 & Alli                & Is alli hungry ?   \\ \hline                                                                                                  
          
\end{tabular}
\caption{Qualitative analysis of rewrites for underspecified queries}
\label{tab:qualitative}
\end{table*}

==> tables/table-ranker.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\newcommand{\mycomment}[1]{}

\mycomment {
\begin{table}[]
\caption{Results for zero-shot retrieval using rewritten queries on BEIR Scifact}
\begin{tabular}{l|l|l}
\textbf{Method}                     & \textbf{NDCG@10}    & \textbf{R@100} \\ \hline
BM25                                & 0.665               & 0.921          \\\hline
tas-b                               & 0.643               & 0.891          \\\hline
RM3+BM25                            & \textbf{0.672}      & 0.918          \\\hline
KL+BM25                             & 0.652               & \textbf{0.922} \\\hline
QE+BM25                             & 0.672               & 0.918          \\\hline
BART(topic-intent) + BM25           & 0.592               & 0.892          \\\hline
BART(topic+paa-target) +BM25        & 0.273               & 0.573          \\\hline
Gpt3 (in context) + bm25            & 0.646 (beats tas-b) & 0.878          \\\hline
Gpt3 (in context) + bm25 (keywords) &                     &                \\\hline
Gpt3 (in context) + tas-b           & 0.602               & 0.858          \\\hline
BART(topic+paa-target) +tas-b       & 0.496               & 0.800          \\\hline
BART(topic-intent) + tas-b          & 0.569               & 0.873          \\\hline
Gpt3 prompt1 + bm25                 & 0.602               & 0.883          \\\hline
Gpt3 prompt1 + tas-b                & 0.570               & 0.862          \\\hline
Gpt3 prompt2 + bm25                 & 0.628               & 0.865          \\\hline
Gpt3 prompt2 + tas-b                & 0.590               & 0.827         \\\hline
\end{tabular}
\end{table}

\\
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Results for zero-shot retrieval using rewritten queries on BEIR Nfcorpus}
\begin{tabular}{lll}
                                    &                  &                                           \\\hline
\textbf{Method}                     & \textbf{NDCG@10} & \textbf{R@100}                            \\\hline
BM25                                & 0.323            & 0.244                                     \\\hline
tas-b                               & 0.319            & 0.280                                     \\\hline
RM3+BM25                            & \textbf{0.328}   & 0.296                                     \\\hline
KL+BM25                             & 0.325            & \textbf{0.296}                            \\\hline
QE+BM25                             & 0.322            & 0.244                                     \\\hline
BART(topic-intent) + BM25           & 0.225            & 0.227                                     \\\hline
BART(topic+paa-target) +BM25        & 0.197            & 0.208                                     \\\hline
Gpt3 (in context) + bm25            & 0.262            & 0.254                                     \\\hline
Gpt3 (in context) + bm25 (keywords) & 0.298            & 0.264                                     \\\hline
Gpt3 (in context) + tas-b           & 0.298            & \textbf{0.284 (better than default)}      \\\hline
BART(topic+paa-target) +tas-b       & 0.220            & 0.228                                     \\\hline
BART(topic-intent) + tas-b          & 0.253            & 0.242                                     \\\hline
Gpt3 prompt1 + bm25                 & 0.283            & 0.274                                     \\\hline
Gpt3 prompt1 + tas-b                & 0.296            & \textbf{0.287(better than default tas-b)} \\\hline
Gpt3 prompt2 + bm25                 & 0.292            & 0.244                                     \\\hline
Gpt3 prompt2 + bm25 (keywords)      & 0.304            & 0.248                                     \\\hline
Gpt3 prompt2 +  tas-b               & 0.300            & 0.274                                      \\\hline
\end{tabular}
\end{table*}
}
